Large Language Models have Intrinsic Self-Correction Ability

Large language models (LLMs) have attracted significant attention for their exceptional abilities in various natural language processing tasks, but they suffer from hallucinations that will cause performance degradation. One promising solution to improve the LLMs' performance is to ask LLMs to revise their answer after generation, a technique known as self-correction. Among the two types of self-correction, intrinsic self-correction is considered a promising direction because it does not utilize external knowledge. However, recent works doubt the validity of LLM's ability to conduct intrinsic self-correction. In this paper, we present a novel perspective on the intrinsic self-correction capabilities of LLMs through theoretical analyses and empirical experiments. In addition, we identify two critical factors for successful self-correction: zero temperature and fair prompts. Leveraging these factors, we demonstrate that intrinsic self-correction ability is exhibited across multiple existing LLMs. Our findings offer insights into the fundamental theories underlying the self-correction behavior of LLMs and remark on the importance of unbiased prompts and zero temperature settings in harnessing their full potential.

==> 4_impact.tex <==
% \section{Experiments}
% \textcolor{red}{delete entire section 5}
% \subsection{Configurations}
% \textcolor{red}{move this before section 2}
% \subsection{Intrinsic Self Correction happens with fair prompt under zero temperature}
% \textcolor{red}{just put the results here. Finish writing later}

% \textcolor{red}{unless otherwise noted, temperature is 0 for non ICLR results}
% \textcolor{red}{Items with * is directly taken from ICLR paper. ICLR Setting: temperature=1}
% See Table \ref{QA_acc}, Table \ref{math_acc}
% \input{Styles/tables/accuracy}
% \subsection{SC ability degrades as temperature rises}
% \input{Styles/tables/temperature}
% \textcolor{red}{Also a chart/image showing number of changed answers increase with temperature}
% \subsection{Universal SC ability under fair prompt}
% \textcolor{red}{highlight different prompt's effect on accuracy. Can split Table 1 and 2, espeically focus on GPT 3.5}

\section{Discussions and Societal Impacts}
Our theoretical analysis and experiment results provide a more fundamental analysis of the intrinsic self-correction ability of large language models. 
We believe that this work will benefit the LLM research community in general by pointing out some preferred experiment settings that shall be used in the future on SC-related works. We also believe that our work will benefit the LLM user community in general by reducing hallucinations in the LLM's response. Reducing LLM's hallucinations might effectively prompt the safety of the online environment, as well as reduce deceptions and fake content generated by LLMs. However, it should also be pointed out that the same technique could be used to generate higher-quality fake content that is harder to be identified.


==> charts/pie_charts.tex <==
\begin{figure}[!ht]
    \centering
    
    % Row 1
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                63.7/C2C, 12.2/C2I, 2.6/I2C, 3.5/I2I-C, 17.9/I2I-NC
            }
        \end{tikzpicture}
        \caption{GPT-3.5 Prompt Set 1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                73.0/C2C, 8.0/C2I, 8.0/I2C, 1.0/I2I-C, 10.0/I2I-NC
            }
        \end{tikzpicture}
        \caption{GPT-4 Prompt Set 1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                63.5/C2C, 2.5/C2I, 3.4/I2C, 3.6/I2I-C, 27.0/I2I-NC
            }
        \end{tikzpicture}
        \caption{Mistral Prompt Set 1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                74.5/C2C, 2.2/C2I, 1.4/I2C, 0.7/I2I-C, 21.2/I2I-NC
            }
        \end{tikzpicture}
        \caption{Phi3 Prompt Set 1}
    \end{subfigure}
    
    % Row 2
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                71.3/C2C, 4.7/C2I, 1.3/I2C, 3.0/I2I-C, 19.6/I2I-NC
            }
        \end{tikzpicture}
        \caption{GPT-3.5 Prompt Set 2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                80.5/C2C, 0.5/C2I, 4.0/I2C, 1.0/I2I-C, 14.0/I2I-NC
            }
        \end{tikzpicture}
        \caption{GPT-4 Prompt Set 2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                65.9/C2C, 0.1/C2I, 1.2/I2C, 2.1/I2I-C, 31.9/I2I-NC
            }
        \end{tikzpicture}
        \caption{Mistral Prompt Set 2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                76.3/C2C, 0.4/C2I, 0.6/I2C, 0.5/I2I-C, 22.3/I2I-NC
            }
        \end{tikzpicture}
        \caption{Phi3 Prompt Set 2}
    \end{subfigure}
    
    % Row 3
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                75.0/C2C, 0.8/C2I, 1.0/I2C, 0.8/I2I-C, 21.7/I2I-NC
            }
        \end{tikzpicture}
        \caption{GPT-3.5 Prompt Set 3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                81.0/C2C, 0.5/C2I, 3.5/I2C, 1.0/I2I-C, 14.5/I2I-NC
            }
        \end{tikzpicture}
        \caption{GPT-4 Prompt Set 3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                65.8/C2C, 0.5/C2I, 1.4/I2C, 1.2/I2I-C, 32.1/I2I-NC
            }
        \end{tikzpicture}
        \caption{Mistral Prompt Set 3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.2\textwidth}
        \centering
        \begin{tikzpicture}
            \pie[radius=1.5, text=legend, explode=0.1]{
                76.7/C2C, 0.1/C2I, 0.3/I2C, 0.2/I2I-C, 22.8/I2I-NC
            }
        \end{tikzpicture}
        \caption{Phi3 Prompt Set 3}
    \end{subfigure}
    
    \caption{Model performance across different prompt sets.}
    \label{fig:model_performance}
\end{figure}


==> tables/models.tex <==
\begin{table}[h]
\centering
\caption{\textcolor{red}{Remove second column or maybe remove whole table?} List of models used and the criteria for sampling the questions from both datasets.}
\begin{tabular}{cc}
\hline
Model                    & Dataset Portion Used \\
\hline

GPT-4-1106-preview       & All questions    \\
GPT-3.5-turbo-0613 / GPT-3.5-turbo-0125       & All questions            \\
Mistral-7B-Instruct-v0.2 & All questions            \\
Phi-3-mini-4k-instruct                     & All questions           \\
Llama3.1-8b-Instruct & All questions \\
\hline
\end{tabular}
\label{models}
\end{table}

==> tables/temperature.tex <==




\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
CommonSense QA      & Before SC & After SC & Difference\\
\hline

GPT3.5 (bias,temp0)                  & 75.68                       & 68.06           & -7.62           \\
GPT3.5 (bias,temp0.3)                & 75.68                       & 63.14          & -12.54           \\
GPT3.5 (bias,temp0.5)                & 75.68                       & 64.05          & -11.63            \\
GPT3.5 (bias,temp0.8)                & 75.68                       & 67.49          & -8.19            \\
GPT3.5 (bias,temp1.0)                & 75.68                       & 66.01    & -9.67  \\
GPT3.5 (bias,temp1.2)                & 75.68                       & 64.78   & -10.9  \\
GPT3.5 (bias,temp1.5)                & 75.68                       & 62.08   & -13.6 \\
\hline
\end{tabular}
\caption{Ablation study on the temperature's effect by fixing first stage. results on temperature, GPT 3.5. \textcolor{red}{maybe convert this to a figure?}}
\label{temperature}
\end{table}
